Finding Critical Scenarios for Automated Driving Systems: A Systematic Literature Review

Scenario-based approaches have been receiving a huge amount of attention in research and engineering of automated driving systems. Due to the complexity and uncertainty of the driving environment, and the complexity of the driving task itself, the number of possible driving scenarios that an ADS or ADAS may encounter is virtually infinite. Therefore it is essential to be able to reason about the identification of scenarios and in particular critical ones that may impose unacceptable risk if not considered. Critical scenarios are particularly important to support design, verification and validation efforts, and as a basis for a safety case. In this paper, we present the results of a systematic literature review in the context of autonomous driving. The main contributions are: (i) introducing a comprehensive taxonomy for critical scenario identification methods; (ii) giving an overview of the state-of-the-art research based on the taxonomy encompassing 86 papers between 2017 and 2020; and (iii) identifying open issues and directions for further research. The provided taxonomy comprises three main perspectives encompassing the problem definition (the why), the solution (the methods to derive scenarios), and the assessment of the established scenarios. In addition, we discuss open research issues considering the perspectives of coverage, practicability, and scenario space explosion.

==> Parts/Jianbo/EuroNCap.tex <==
Euro NCAP (European New Car Assessment Program) is a well-known organization for car safety performance assessment, it provides a safety performance assessment by means of rating. Euro NCAP mainly provides testing and evaluation procedures for "passive safety technology" and "active safety technology". With the development of autonomous driving technology, Euro NCAP is focusing more and more on the evaluation of "active safety technology". The active safety technologies include AEB (Autonomous Emergency Braking) - City, AEB - Vulnerable Road User, AEB - Inter-Urban, Speed Assist System, SLF (Speed Limit Function, SLIF (Speed Limit Infomation Function), ISA (Intelligent Speed Assistance), Intelligent ACC (Adaptive Cruise Control), Lane Support System, ELK (Emergency Lane Keeping), LKA(Lane Keeping Assist) and LDW(Lane Departure Warning). 

==> Parts/Jianbo/ISO3450.tex <==
The ISO/TC22/SC33/WG9 3450X were started from year 2018. The main target of this group is to create standard for the implementation of the definition of terms, process framework, database, design and operation scope, test evaluation and other international standards related to autonomous driving test scenarios. The detailed sub-standards are:

ISO 34501: Road Vehicles - Terms and Definitions of Test Scenarios for Automated Driving Systems

ISO 34502: Road Vehicles - Engineering Framework and Process of Scenario-based Safety Evaluation

ISO 34503: Road Vehicles - Taxonomy for Operational Design Domain for Automated Driving Systems  

ISO 34504: Road Vehicles - Scenario Attributes and Categorization

ISO PWI: Road Vehicles – Evaluation of Test Scenario


==> Parts/Jianbo/OpenX.tex <==
The OpenX standard released by ASAM (The Association for Standards in Automation and Measurement Systems) has received widespread attention worldwide. 
In the process of promoting the implementation of autonomous driving, simulation is currently an important way for testing and verification internationally. However, in the actual development process, the data formats and interfaces used by vehicle manufacturers, suppliers and simulation tool vendors are diverse, so it is imperative to develop a unified simulation format standard. Since ASAM launched the OpenX series of format standards, more than 100 companies around the world have participated in the development of this series of standards, including major OEMs and Tier 1 suppliers in Europe, America and Japan.

At present, in the field of ASAM simulation verification, the OpenX series standards mainly include OpenDRIVE, OpenSCENARIO, Open SimulationInterface (OSI), OpenLABEL and OpenCRG in five major segments. The OpenXOntology and OpenODD projects were just started in 2020. In the overall process of simulation testing, OpenDRIVE and OpenSCENARIO are unified for different data formats of simulation scenarios. The OpenDRIVE standard defines the description method of static scenes. The content defined by the OpenSCENARIO standard mainly covers dynamic scene descriptions, including information such as the position and speed of the main vehicle and information about other traffic participants. OpenLABEL will give a unified calibration method for raw data and scenarios. OpenOSI connects autonomous driving functions with simulation tools and integrates various sensors at the same time. OpenCRG realizes the physical information of road surface and static OpenCRG enables the interaction between physical road information and static road scenes. The goal of the ASAM OpenX Ontology project is to define an architecture for an ontology that acts as a clear and unambiguous specification of the shared domain model of road traffic for the OpenX domain. In addition, the project will provide implementations of core modules of the ontology for describing concepts and relationships of entities and environments relevant to road traffic. ASAM OpenODD is a representation of the abstract ODD specification in a more well-defined syntax and semantics which enables machines to interpret and perform the required analysis. Additionally, the OpenODD specification shall be measureable and verifiable for the attributes it specifies.

==> Parts/Jianbo/UNECE.tex <==
The intention of the UNECE ALKS Regulation is to lay down uniform provisions for the approval of vehicles equipped with an Automated Lane Keeping System (ALKS). 

==> Parts/Jianbo/required_databases.tex <==
% \begin{table}[!t]
% \caption{Different purposes and applications of data-driven approach}
% \label{tabrealdata}
% \centering
% \begin{tabular}{|C{2.5cm}|L{9cm}|}
% \hline
% \textbf{Data source} &  \multicolumn{1}{c|}{\textbf{Purpose}} \\ 
% \hline
% \multirow{2}{2.5cm}{\centering Real data}
% & Using real data to generate the distributions of scenario parameters
% for scenario extraction or function assessment \& validation (e.g. MonteCarlo simulation) ~\cite{DeGelder2017a,Vehicles2020,Feng2019b,Wagner2018,Erdogan2019,Klitzke2019} \\
% \cline{2-2}
% & Using real data for human-driving behaviour modelling for function assessment or safety evaluation ~\cite{Roesener2016,Zhao2015b,Wang2018a,Kuefler2017,Notz2019}\\
% \hline
% Traffic flow data & Using real traffic data to calibrate and validate driver behaviour model and simulation model ~\cite{Zhao2016,Caliendo2012} \\ 
% \hline
% Accident database & Using accident database for scenario creation ~\cite{Lenard2014a,Marschner2015} \\ 
% \hline
% \end{tabular}
% \end{table}

In this section we present the results about how the real world data i.e. data-driven approach are used in the surveyed papers. To support the activities of verification and validation (V\&V) of ADAS and automated-driving system several data sources are used. These sources could be mainly categorized into three domains: virtual, verbal and real. Virtual data is the data source which comes out via virtual method e.g. simulation or driving simulator. Verbal means the data or the knowledge from expert. Real denotes the approach which utilizes the data source from real world. We summarized the real data into the following three categories: real data, traffic flow data and accident database. The real data includes real-driving data, FOT (field operational test) and naturalistic driving data. Accident database includes the accident report database source and research studies. Table \ref{tabrealdata} shown the different purposes and applications of data-driven approach. 

\textbf{Real data:} As shown in the table the main usages of the real data from the surveyed papers are using real data to approximate the distributions of scenario parameters for scenario sampling or function assessment \& validation and using real data for human-driving behaviour modelling for function assessment or safety evaluation. The authors in~\cite{DeGelder2017a} used the naturalistic driving data to generate scenarios and test cases. These test cases were furthermore used for Monte-Carlo simulation for critical scenario finding and eventually function assessment. In ~\cite{Vehicles2020} and ~\cite{Feng2019b} the real driving data were used to derive and support the construction of a surrogate model, which is used to indicate the safety performance in the lane-change scenario. The authors in ~\cite{Erdogan2019}~\cite{Klitzke2019} presented methods to extract scenarios from the time- series states of the real-world measurement data. In ~\cite{Wagner2018} the authors used the real driving data to derive the distributions of the parameters, which were later used for a Monte-Carlo simulation to determine the possible evolution of scenario.
In ~\cite{Roesener2016,Zhao2015b,Wang2018a} real human driving behaviour data was used as reference for criticality and function assessment. The authors in ~\cite{Kuefler2017,Notz2019} utilized the real data to train the behavior models for traffic objects for function assessment.

\textbf{Traffic flow data:} In ~\cite{Zhao2016,Caliendo2012} the authors used real traffic data to calibrate and validate driver behaviour model, which was furthermore used in simulation for the safety evaluation. 

\textbf{Accident database:} Authors in ~\cite{Lenard2014a,Marschner2015} analysed the accident database and research studies, summarised the important and relevant information. Afterwards representative scenarios were created for the function validation and testing.  

==> Parts/Kaige/coverage.tex <==
% this part is not included in the article
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Coverage plays a pivotal role in the scenario-based testing, since the validation of AD/ADAS functions in terms of safety are highly determined by the requirements and assumptions proposed during the test phases. As the real-world tests are not scalable to sufficiently cover the variant system environment, the satisfaction of the testing coverage to a great extent can ensure the integrity of validation through covering the vast majority of cases occurring on the real road. In this study, we consider mechanisms for coverage applied in the scenario space exploration, which is shown in Figure~\ref{fig:coverage_mechanism}.

\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{Images/coverage_figure_Kaige.pdf}
\caption{mechanisms for coverage in scenario space exploration} \label{fig:coverage_mechanism}
\end{figure*}

%The coverage metrics embody the requirements and levels on the evaluation of the testing. It can influence the  and is largely depend on  
We define the coverage metrics in three different types: ~(1) N-wise, which is the coverage pattern applied in CT ~(2) functional coverage, examined with particular characteristics based on the functionalities and approaches employed in the test case generation, and ~(3) other methods, which exists but have not been studied in this survey. N-wise requires identifying and evaluating every possible pair of \emph{N} parameters with their all possible values, under the assumption that each variable is orthogonal. N-wise is a way to ensure the test coverage in black-box tests, which is widely used in the combinatorial testing, providing a way to circumvent exhaustive testing and save test effort \cite{ponn2019towards, Li2020, Tuncali2018, tuncali2019requirements, Gao2019}. Functional coverage method is a structural coverage metrics at the software architectural level as defined by ISO 26262 \cite{ISO26262}. Test automation tool, such as Vitaq \cite{Khastgir2017}, can be utilized to achieve functional coverage based on defined use case requirements. To this end, some other standard coverage metrics, such as statement coverage, branch coverage and call coverage can be fulfilled in a similar way.

Diversity is a means to evaluate coverage over different test cases in the sense of assessing the distinctiveness of each scenario. It helps to check the redundancies in a set of test scenarios regarding both scenario and criticality space. The scenario space stands for the parameter space, where the values of variables are specified at the initialization stage of a test. Besides, the criticality space reflects all possible results in test cases based on simulation and evaluation. Both spaces' inspections are favourable since the probability of large areas not being exposed or samples being too close together can be minimized. For the scenario space, it is desired to maximize the distance among different test points with the intent to guarantee the samples are homogeneously spread \cite{batsch2019performance}. Different measures to estimate distances can be applied, such as Voronoi interpolation \cite{Gladisch2019}, which is used when sampling in a two-dimensional space to ensure no tests exist in close Euclidean distance. Moreover, various sampling methods, such as Latin Hypercube Sampling \cite{batsch2019performance}, can improve the diversity of samples compared to random sampling, which divides each parameter into intervals to ensure the parameter space is evenly covered. The assessment in the criticality space depends on the prior knowledge of the system under test. \cite{Mullins2018} assumes that the behaviour of the system is deterministic under one scenario configuration. The performance is evaluated in a scoring space, where each dimension is a performance metric. It takes a set of samples as input and returns the estimated diversity (i.e., the mean distance) on the scoring space of the input samples.

Local minimums are investigated mainly in the optimization and learning-based testing use cases. It is worth noting that, in some instances, finding the global minimum is the objective rather than local minimums \cite{Beglerovic2018, pop00261}. However, in those applications, local minimums are stilled discovered during iterations for training, and as such we incorporate them in this category. In heuristic approaches, such as genetic algorithm \cite{kluck2019performance, pop00010, cutrone2018framework}, instead of searching the global optimum, a solution which detects critical cases reaching a particular threshold value is the target. Similar ideas can be found in \cite{gangopadhyay2019identification}, where multiple local minimums are identified, corresponding to all the test cases causing failures.


% - reason about the coverage
%     consider the commonality of the scenarios
%         qualitative consideration
%             surrogate model \cite{Mullins2018,Nabhan2019a}
%             heuristics (e.g., less severe means more common) \cite{Tuncali2018,Batsch2019a}
%          quantitative consideration
%             distribution of parameters from real-data \cite{Feng2019b,DeGelder2017a}
%             constraints on the parameters
%             Likelihood of exposure of each scenario from traffic/accident databases 
            
%     do not consider the commonality of the scenarios
%         Combinatorial test \cite{Li2020,Tuncali2018}
%         Systemetic analysis \cite{CV-HAZOP,koopman2019,Zhou2017a,weber2018}
%         exhaustive search (e.g., model checking) \cite{Damm2018a}
    
%     mention the SOTIF figure        
    
    
    % real world test are not scalable to sufficiently cover the variant system environment.

==> Parts/Naveen/UL4600.tex <==
The UL4600 was developed as a joint collaboration between Underwriters Laboratories, and Edge Case Research with a large and diverse technical panel comprising representatives from Industry and Academia. The focus of this standard on building and evaluating the safety argumentation of an fully automated ADS feature. UL4600 provides several normative clauses with "prompts" that are classified into Mandatory, Required, Highly Recommended, and Recommended categories to indicate the relative importance of the particular prompts in fulfilling the clause it is linked to.

As a standard for safety arguementation for fully automated systems, with a self-professed goal of being aiming to be technology neutral and non-prescriptive, the UL4600 does not favor any particular scenario description language or a formal model of describing the environmental factors. Instead the standard mandates the definition and use of a a complete ODD definition with traceability to the ODD-dependent aspects of the safety case, requires the inclusion of environmental factors and a defined scenario description languages, and highly recommends the positive, negative and neutral enumerations of the ODD. Thus scenarios are addressed in terms of their relevance to the ODD, including requirements to monitor and formalization of strategies to handle violations i.e. departures from the ODD. 

The UL4600 further, mandates the definition of certain classes of components that must be included in an ODD definitions thereby mandating the use of static objects, actors, environmental conditions, and operational conditions, along with the definition of behavioral rules and the measurement of the interaction of the ADS feature with the ODD using Safety Performance Indicators.  Thus, without explicitly requiring a structure in the constructions of the scenarios for an ADS, or the detailed enumeration of all the classes, the standard provides a basic framework of proto-classes of components and their interaction. The assessment of criticality of the scenarios that should emerge from this framework, and the concreteness of scenarios needed to test the safety goals, is left to be chosen by the designer of the ADS feature on the basis of guidance from other related standards specialized towards functional and system safety. 

==> Tables/clusters.tex <==
\begin{table}
\centering
\caption{Primary studies under each cluster of methods}
\label{tab:clusters}
\begin{tabular}{|l|l|} 
\hline
\multicolumn{1}{|c|}{ \textbf{Cluster} }                                                                     & \multicolumn{1}{c|}{\textbf{Primary Study} }  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Exploring the scenario space \\without motion profiles \end{tabular}              &                           34                    \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Exploring the scenario space\\\textasciitilde{}with motion profiles \end{tabular} &                                               \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Finding critical scenes for \\CV-based functions \end{tabular}                    &                                               \\ 
\hline
Formal methods                                                                                               &                                               \\ 
\hline
Deductive~reasoning                                                                                          &                                               \\ 
\hline
Inductive reasoning                                                                                          &                                               \\ 
\hline
Others                                                                                                       &                                               \\
\hline
\end{tabular}
\end{table}

==> notes.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.
% However, the Computer Society has been known to put floats at the bottom.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.

==> sections/Notes.tex <==



As a complementary standard of the automotive functional safety standard ISO 26262, ISO/PAS 21448 focuses on the Safety Of The Intended Functionality (SOTIF). It extends the ISO 26262 methodology by considering more sources of harm. This section only introduces the parts related to CSI methods.

In ISO 26262, functional safety is defined as the absence of unreasonable risk due to hazards caused by malfunctioning behavior of E/E systems, where a malfunctioning behavior refers to a behavioral deviation from the design intent. It assumes that the design intent is safe, and deviations are caused by either systematic faults or random hardware faults. However, this assumption is not always valid for ADS and ADAS for two reasons: 
\begin{enumerate}
    \item Due to the openness of the driving environment, specifications of AD functions may not be sufficient. Consequently, some unidentified edge cases may lead to safety problems.
    \item Deviation from the intended functionality can also stem from inevitable performance limitations of some advanced functions due to the complexity or the inductive nature (e.g., learning-based methods) of the employed algorithm.
\end{enumerate}
 
In ISO/PAS 21448, these insufficient specifications and performance limitations are defined as functional insufficiency, which may lead to a hazardous behavior on the system level (e.g., improper estimation of the distance with the front vehicle). As shown in Fig. \ref{fig:SOTIF}, a hazardous behavior may propagate to a hazard (i.e., an unintended behavior on the vehicle level, e.g., an unintended acceleration). Each functional insufficiency is associated with one or more external triggering conditions. If a hazard happens in a safety-critical operational situation (e.g., the ego vehicle is running on a highway with small distance to the front vehicle), there is a high risk of a harm, especially when the involved person (e.g., the driver for a L2 or L3 AD system) cannot react properly. Triggering conditions and hazard operational condition are two major components of a safety-critical scenario. Therefore, an unknown critical scenario can stem from either an unknown triggering condition or an unknown safety-critical operational situation. In addition, Annex B2 of ISO/PAS 21448 further assumes that a scenario condition/situation can be modeled as a combination of several scenario factors (e.g., heavy rain, glare, slippery road surface, a sudden cut in on another vehicle etc). Under this assumption, an unknown critical scenario can be attributed to either an unknown scenario factor or an unknown combination of known scenario factors. 

\begin{figure*}[!t]
\centering
\includegraphics[width=0.85\textwidth]{SOTIF_assumption}
\caption{Sources of harm according to ISO 26262, ISO/PAS 21448 and SAE J3016} 
\label{fig:SOTIF}
\end{figure*}

Not all scenarios containing one or more triggering conditions as critical scenarios. The triggered hazardous behavior may not propagate to a vehicle-level hazard owning to the resilience of the system. In addition, the hazard propagated from the triggering conditions may not lead to an accident without a hazardous operation condition. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{sources_unknown_CS}
\caption{Sources of unknown critical scenarios} 
\label{fig:source_unknown_CS}
\end{figure}




Usage of traffic Simulator (e.g., SUMO)
    generate behaviors of vehicles
        incomplete behaviors
        unrealistic behaviors [calibrate SUMO with real data]

Usage of driving Simulators (e.g., PreScan)
    calculate criticality measures
        false positive
        false negative [thresholding]
    validate the identified critical scenarios
        false positive
        false negative
    state inference (cluster 2)
        totally wrong result because of accumulative error
    scene improvisation (for computer vision)
        cannot reflect real camera physics

•	Data quality (data was used for critical scenario finding)
    Usage of data:
    accident data 
        - to find typical critical scenario
        - use as test case
    naturalistic driving data
        - approximate parameter distribution from real --> how to ensure the derived distribution meets the distribution in ODD data 
        - safety assessment
    traffic data
        - use traffic data in simulation to extract more concrete crash scenarios
        
        
        
General comments: 
- past tense or presense for referring to what has/is done in different papers?
- Article or paper when referring to other work?
- SUT or SOI?
- Harmonize usage of : in section titles...
- Maybe add some short discussion of ISO 5083 and ISO TS 4804 in the second section?


better to provide a list of simulation types

==> sections/Relevant_industrial_standards.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relevant Industrial Standards}
\label{sec:standards}

\subsubsection{ISO/PAS 21448}
\label{sec:SOTIF}
As a complementary standard of the automotive functional safety standard ISO 26262, ISO/PAS 21448 focuses on the Safety Of The Intended Functionality (SOTIF). It extends the ISO 26262 methodology by considering more sources of harm. This section only introduces the parts related to CSI methods.

In ISO 26262, functional safety is defined as the absence of unreasonable risk due to hazards caused by malfunctioning behavior of E/E systems, where a malfunctioning behavior refers to a behavioral deviation from the design intent. It assumes that the design intent is safe, and deviations are caused by either systematic faults or random hardware faults. However, this assumption is not always valid for ADS and ADAS for two reasons: 
\begin{enumerate}
    \item Due to the openness of the driving environment, specifications of AD functions may not be sufficient. Consequently, some unidentified edge cases may lead to safety problems.
    \item Deviation from the intended functionality can also stem from inevitable performance limitations of some advanced functions due to the complexity or the inductive nature (e.g., learning-based methods) of the employed algorithm.
\end{enumerate}

In ISO/PAS 21448, these insufficient specifications and performance limitations are defined as functional insufficiency, which may lead to a hazardous behavior on the system level (e.g., improper estimation of the distance with the front vehicle). As shown in Fig. \ref{fig:SOTIF}, a hazardous behavior may propagate to a hazard (i.e., an unintended behavior on the vehicle level, e.g., an unintended acceleration). Each functional insufficiency is associated with one or more external triggering conditions. If a hazard happens in a safety-critical operational situation (e.g., the ego vehicle is running on a highway with small distance to the front vehicle), there is a high risk of a harm, especially when the involved person (e.g., the driver for a L2 or L3 AD system) cannot react properly. Triggering conditions and hazard operational condition are two major components of a safety-critical scenario. Therefore, an unknown critical scenario can stem from either an unknown triggering condition or an unknown safety-critical operational situation. In addition, Annex B2 of ISO/PAS 21448 further assumes that a scenario condition/situation can be modeled as a combination of several scenario factors (e.g., heavy rain, glare, slippery road surface, a sudden cut in on another vehicle etc). Under this assumption, an unknown critical scenario can be attributed to either an unknown scenario factor or an unknown combination of known scenario factors. 

\begin{figure*}[!t]
\centering
\includegraphics[width=0.85\textwidth]{SOTIF_assumption}
\caption{Sources of harm according to ISO 26262, ISO/PAS 21448 and SAE J3016} 
\label{fig:SOTIF}
\end{figure*}

Not all scenarios containing one or more triggering conditions as critical scenarios. The triggered hazardous behavior may not propagate to a vehicle-level hazard owning to the resilience of the system. In addition, the hazard propagated from the triggering conditions may not lead to an accident without a hazardous operation condition. 


\subsubsection{UL 4600}
\input{Parts/Naveen/UL4600}

%\subsubsection{ISO/TR 4804}
%\input{Parts/Jianbo/TR 4804}

\subsubsection{EuroNCap}
\input{Parts/Jianbo/EuroNCap}

\subsubsection{ASAM OpenX}
\label{sec:OpenX}
\input{Parts/Jianbo/OpenX}

\subsubsection{ISO 3450X}
\input{Parts/Jianbo/ISO3450}

\subsubsection{PAS 1883}
\input{Parts/Jianbo/PAS1883}

\subsubsection{UNECE ALKS Regulation}
\input{Parts/Jianbo/UNECE}
